PEARLS: NuSTAR and XMM-Newton Extragalactic Survey of the JWST North Ecliptic Pole Time-Domain Field IV: X-Ray Variability Analysis

NuSTAR and XMM-Newton have observed the James Webb Space Telescope (JWST) North Ecliptic Pole (NEP) Time-Domain Field (TDF) for almost five contiguous years starting in 2019. In that time, the NEP X-ray survey has accumulated 3.5 Ms and 228 ks of quasi-simultaneous NuSTAR and XMM-Newton observations, respectively. This paper presents variability results for the 112 NuSTAR and 453 XMM-Newton sources detected in this field, based solely on the X-ray photometric data. Four NuSTAR sources and 11 XMM-Newton sources varied in at least one band at >=99% confidence. The sources with redshift measurements show a relationship between luminosity and variability with 74% of variable sources brighter than 5x the sensitivity limit of the survey. This is supported by about 1/3 of sources with more than 400 counts detected being variable and only 4 sources with fewer counts showing variability. Variability timescales are not well determined, but variability amplitude tends to be larger on longer timescales.

==> nustar_catalog.tex <==
1&J172401+6600.5&2&10&375&261.0062&66.0085&0.8918&\no&Q&5.97e$-$01&8.87e$-$01&7.68e$-$01&11.58& 0.14&255 \\
2&J172129+6551.2&14&23&\no&260.3713&65.8540&\no&\no&N&9.01e$-$01&9.78e$-$01&7.54e$-$01&\no&\no&187 \\
3&J172246+6544.3&19&38&227&260.6944&65.7387&\no&\no&N&3.39e$-$01&9.76e$-$01&5.16e$-$01&11.20& 0.10&437 \\
4&J172328+6559.2&20&12&318&260.8686&65.9867&1.4252&\no&Q&9.88e$-$02&7.01e$-$01&2.65e$-$01&11.00& 0.71&192 \\
5&J172316+6556.7&21&14&305&260.8167&65.9464&0.4949&\no&G&1.69e$-$01&3.13e$-$01&6.63e$-$02&11.31&$-$2.10&350 \\
6&J172236+6555.6&22&16&218&260.6527&65.9271&\no&0.56&N&9.85e$-$01&9.94e$-$01&9.53e$-$01&\no&\no&406 \\
7&J172141+6555.1&24&71&108&260.4235&65.9190&0.5233&\no&Q&9.58e$-$01&6.38e$-$01&6.41e$-$01&10.85& 0.32&451 \\
8&J172403+6550.6&26&31&378&261.0156&65.8439&\no&\no&N&6.89e$-$01&8.92e$-$01&7.97e$-$01&10.65&$-$1.12&193 \\
9&J172313+6547.8&29&28&299&260.8072&65.7975&1.4411&\no&N&2.66e$-$10&2.14e$-$04&6.66e$-$16&11.66& 2.71&4412 \\
10&J172145+6550.3&30&26&122&260.4383&65.8392&\no&\no&N&8.21e$-$01&7.85e$-$01&8.28e$-$01&\no&\no&202 \\
11&J172416+6548.9&31&54&406&261.0688&65.8152&0.3759&\no&G&9.55e$-$01&9.94e$-$01&9.91e$-$01&11.25&$-$0.75&367 \\
12&J172209+6545.3&35&34&160&260.5379&65.7561&\no&\no&N&9.90e$-$01&9.23e$-$01&9.74e$-$01&\no&\no&246 \\
13&J172219+6544.3&36&32&193&260.5797&65.7385&1.0190&\no&Q&5.08e$-$01&9.26e$-$01&9.28e$-$01&10.99& 0.51&248 \\
14&J172408+6543.9&37&42&379&261.0350&65.7326&\no&0.46&N&8.81e$-$01&9.96e$-$01&9.88e$-$01&10.96& 0.64&183 \\
15&J172259+6554.6&41&19&266&260.7465&65.9101&\no&\no&N&7.27e$-$01&9.94e$-$01&8.15e$-$01&11.31& 0.43&332 \\
16&J172233+6550.9&43&25&213&260.6384&65.8485&1.3369&\no&Q&4.96e$-$01&2.94e$-$01&3.65e$-$01&11.14& 0.51&443 \\
17&J172356+6549.7&45&68&367&260.9855&65.8289&\no&1.75&N&9.84e$-$01&9.04e$-$01&9.72e$-$01&11.18& 0.31&530 \\
18&J172241+6539.7&48&69&\no&260.6718&65.6629&\no&\no&N&9.33e$-$01&8.64e$-$01&8.59e$-$01&\no&\no&191 \\
19&J172306+6551.3&53&72&279&260.7752&65.8562&0.8846&\no&Q&5.15e$-$01&4.05e$-$01&8.18e$-$02&10.35&$-$0.91&1043 \\
20&J172333+6548.9&54&55&327&260.8888&65.8167&0.7791&\no&G&8.99e$-$02&7.52e$-$01&8.38e$-$01&11.25&$-$0.53&365 \\
21&J172143+6546.1&55&56&111&260.4313&65.7688&0.7813&\no&Q&2.94e$-$01&8.83e$-$01&4.03e$-$01&10.93& 0.96&1067 \\
22&J172157+6544.3&57&59&148&260.4916&65.7390&\no&\no&N&9.34e$-$01&9.28e$-$01&9.63e$-$01&\no&\no&197 \\
23&J172241+6542.7&58&75&222&260.6730&65.7127&0.1791&\no&G&1.72e$-$03&1.23e$-$01&2.39e$-$04&10.72&$-$0.22&1526 \\
24&J172207+6603.5&1&\no&\no&260.5307&66.0599&\no&\no&N&4.18e$-$02&5.76e$-$01&4.29e$-$02&\no&\no&44 \\
25&J172227+6558.8&3&\no&207&260.6156&65.9802&\no&\no&S&7.49e$-$01&5.53e$-$01&8.59e$-$01&11.19& 2.24&100 \\
26&J172259+6558.1&4&\no&\no&260.7499&65.9687&\no&\no&N&5.72e$-$01&9.52e$-$01&5.49e$-$01&\no&\no&112 \\
27&J172144+6557.6&5&\no&\no&260.4348&65.9613&\no&\no&N&4.14e$-$01&9.29e$-$01&6.15e$-$01&\no&\no&74 \\
28&J172205+6557.2&6&\no&154&260.5220&65.9540&\no&\no&N/A&4.46e$-$01&8.81e$-$01&5.09e$-$01& 9.38& 1.10&274 \\
29&J172152+6556.0&7&\no&134&260.4687&65.9348&0.2699&\no&G&9.38e$-$01&8.07e$-$01&7.07e$-$01&11.27& 2.07&79 \\
30&J172229+6555.4&8&\no&208&260.6229&65.9235&\no&\no&N/A&8.99e$-$01&8.71e$-$01&6.33e$-$01&10.83& 3.09&91 \\
31&J172445+6552.9&9&\no&\no&261.1881&65.8817&\no&\no&N&4.79e$-$01&3.00e$-$01&6.28e$-$02&\no&\no&66 \\
32&J172210+6553.2&10&\no&172&260.5447&65.8878&\no&\no&N/A&8.95e$-$01&9.81e$-$01&5.38e$-$01&10.11&$-$0.32&98 \\
33&J172255+6553.4&11&\no&254&260.7318&65.8902&0.6007&\no&Q&9.92e$-$01&9.96e$-$01&9.96e$-$01& 8.82&$-$0.94&136 \\
34&J172151+6552.7&12&\no&129&260.4662&65.8795&\no&\no&N/A&1.00e+00&9.66e$-$01&9.73e$-$01&10.66& 1.64&135 \\
35&J172308+6552.3&13&\no&286&260.7837&65.8725&\no&\no&N/A&9.89e$-$01&6.58e$-$01&8.82e$-$01&\no&\no&146 \\
36&J172209+6547.4&15&\no&163&260.5392&65.7902&\no&\no&N/A&9.23e$-$01&9.88e$-$01&9.46e$-$01&11.21& 0.13&113 \\
37&J172424+6546.2&16&\no&\no&261.1035&65.7706&\no&\no&N&6.31e$-$01&9.11e$-$01&6.91e$-$01&\no&\no&66 \\
38&J172354+6543.4&17&\no&\no&260.9785&65.7236&2.2508&\no&Q&5.77e$-$01&8.34e$-$01&2.94e$-$01&\no&\no&90 \\
39&J172136+6543.2&18&\no&\no&260.4039&65.7209&\no&\no&N&9.72e$-$01&8.44e$-$01&8.37e$-$01&\no&\no&60 \\
40&J172159+6554.4&23&\no&144&260.4959&65.9075&0.4949&\no&G&9.29e$-$01&9.93e$-$01&9.66e$-$01&\no&\no&125 \\
41&J172446+6551.5&25&\no&\no&261.1945&65.8592&\no&\no&N/A&1.14e$-$01&4.06e$-$01&5.04e$-$02&\no&\no&114 \\
42&J172205+6550.0&27&\no&\no&260.5236&65.8345&0.5233&\no&Q&8.64e$-$01&9.91e$-$01&8.47e$-$01&\no&\no&114 \\
43&J172351+6550.2&28&\no&356&260.9657&65.8369&\no&\no&N&8.97e$-$01&9.55e$-$01&8.26e$-$01&\no&\no&206 \\
44&J172246+6548.4&32&\no&229&260.6956&65.8082&1.4411&\no&Q&7.12e$-$01&9.92e$-$01&8.53e$-$01&\no&\no&157 \\
45&J172427+6548.6&33&\no&\no&261.1155&65.8101&\no&\no&N/A&3.04e$-$01&9.30e$-$01&3.56e$-$01& 8.52&$-$2.76&183 \\
46&J172332+6546.8&34&\no&325&260.8855&65.7817&0.3759&\no&G&8.79e$-$01&9.97e$-$01&8.61e$-$01&\no&\no&82 \\
47&J172401+6538.1&38&\no&\no&261.0063&65.6355&0.4031&\no&G&3.01e$-$02&2.13e$-$01&7.23e$-$02& 8.12&$-$0.36&49 \\
48&J172248+6600.8&39&\no&241&260.7026&66.0144&\no&\no&N&9.27e$-$01&1.17e$-$01&7.14e$-$01&\no&\no&65 \\
49&J172357+6555.3&40&\no&\no&260.9911&65.9230&1.0190&\no&Q&9.39e$-$01&3.13e$-$01&3.26e$-$01& 4.88&$-$5.09&126 \\
50&J172413+6552.2&42&\no&\no&261.0543&65.8703&\no&\no&N&1.00e+00&8.27e$-$01&9.71e$-$01&\no&\no&111 \\
51&J172252+6550.7&44&\no&\no&260.7187&65.8451&\no&\no&N&1.00e+00&7.13e$-$01&9.01e$-$01&\no&\no&173 \\
52&J172304+6546.4&46&\no&281&260.7691&65.7741&\no&\no&N/A&5.50e$-$01&8.79e$-$01&7.92e$-$01& 9.35&$-$2.17&264 \\
53&J172304+6549.3&47&\no&\no&260.7672&65.8219&\no&\no&N&9.43e$-$01&8.44e$-$01&8.09e$-$01&\no&\no&241 \\
54&J172355+6555.9&49&\no&\no&260.9828&65.9325&\no&\no&N&9.71e$-$01&6.72e$-$01&4.81e$-$01&\no&\no&103 \\
55&J172312+6555.7&50&\no&\no&260.8019&65.9298&\no&\no&N/A&9.38e$-$01&9.89e$-$01&9.85e$-$01&11.20& 0.53&114 \\
56&J172213+6556.9&51&\no&183&260.5573&65.9486&0.6339&\no&Q&9.52e$-$01&6.07e$-$01&6.04e$-$01&\no&\no&162 \\
57&J172317+6553.7&52&\no&\no&260.8238&65.8957&\no&\no&N/A&5.74e$-$01&9.05e$-$01&6.42e$-$01&11.24&$-$0.58&120 \\
58&J172215+6545.8&56&\no&\no&260.5662&65.7643&\no&\no&N&9.56e$-$01&8.72e$-$01&9.13e$-$01&\no&\no&82 \\
59&J172313+6542.3&59&\no&\no&260.8075&65.7052&\no&\no&N&9.33e$-$01&6.89e$-$01&8.41e$-$01&\no&\no&111 \\
60&J172254+6541.9&60&\no&248&260.7262&65.6990&0.8846&\no&Q&7.38e$-$01&7.51e$-$01&6.72e$-$01&10.15& 0.09&105 \\
61&J172143+6606.2&\no&1&\no&260.4301&66.1048&\no&\no&N&5.09e$-$01&9.19e$-$02&4.73e$-$02&\no&\no&69 \\
62&J172454+6605.5&\no&2&\no&261.2256&66.0922&\no&\no&N&\no&\no&\no&\no&\no&50 \\
63&J172151+6604.8&\no&3&\no&260.4659&66.0817&0.9130&\no&Q&8.32e$-$02&4.32e$-$02&5.17e$-$03&10.03& 0.63&181 \\
64&J172450+6603.8&\no&4&\no&261.2084&66.0642&\no&\no&N&5.85e$-$02&5.34e$-$01&2.78e$-$01&\no&\no&54 \\
65&J172205+6604.0&\no&5&\no&260.5217&66.0682&\no&\no&N&8.91e$-$01&5.64e$-$01&4.89e$-$01&10.71& 2.46&89 \\
66&J172237+6602.8&\no&6&\no&260.6549&66.0473&\no&\no&N&5.82e$-$01&2.53e$-$01&3.16e$-$01&\no&\no&58 \\
67&J172307+6602.6&\no&7&\no&260.7794&66.0440&\no&\no&N&5.00e$-$01&5.42e$-$01&2.47e$-$01&\no&\no&68 \\
68&J172412+6602.3&\no&8&\no&261.0518&66.0399&\no&\no&N&4.03e$-$01&9.25e$-$01&5.51e$-$01&\no&\no&87 \\
69&J172426+6602.1&\no&9&\no&261.1106&66.0350&\no&\no&N&7.26e$-$01&8.07e$-$01&5.44e$-$01&\no&\no&74 \\
70&J172148+6559.8&\no&11&127&260.4506&65.9976&\no&0.63&N&7.83e$-$01&7.60e$-$01&6.71e$-$01&11.41&$-$0.46&109 \\
71&J172208+6557.0&\no&13&161&260.5368&65.9514&\no&\no&N&7.58e$-$01&9.65e$-$01&5.30e$-$01&10.84&$-$0.27&130 \\
72&J172043+6557.0&\no&15&\no&260.1800&65.9509&\no&\no&N&9.35e$-$01&8.72e$-$01&9.90e$-$01&\no&\no&92 \\
73&J172450+6555.4&\no&17&\no&261.2084&65.9242&\no&\no&N&9.52e$-$02&6.93e$-$02&5.20e$-$03&\no&\no&84 \\
74&J172343+6555.7&\no&18&\no&260.9322&65.9286&0.3768&\no&G&5.76e$-$01&8.64e$-$01&2.17e$-$01&\no&\no&133 \\
75&J172154+6555.7&\no&20&\no&260.4752&65.9294&0.2699&\no&G&7.09e$-$01&7.93e$-$01&3.63e$-$01&\no&\no&105 \\
76&J172251+6553.4&\no&21&237&260.7166&65.8917&0.0011&\no&G&6.52e$-$01&8.67e$-$01&7.67e$-$01& 5.60&$-$10.14&88 \\
77&J172431+6551.6&\no&22&\no&261.1308&65.8609&\no&\no&N&9.97e$-$01&9.14e$-$01&7.44e$-$01&\no&\no&78 \\
78&J172452+6551.1&\no&24&238&261.2176&65.8525&\no&\no&N&7.89e$-$01&8.64e$-$01&6.30e$-$01&\no&\no&102 \\
79&J172247+6550.3&\no&27&\no&260.6969&65.8391&\no&1.46&N&6.40e$-$01&8.05e$-$01&2.90e$-$01&\no&\no&110 \\
80&J172407+6549.8&\no&29&383&261.0322&65.8303&\no&\no&N&9.60e$-$01&8.47e$-$01&6.40e$-$01&\no&\no&97 \\
81&J172210+6548.0&\no&30&\no&260.5440&65.8005&\no&\no&N&8.06e$-$01&9.36e$-$01&9.76e$-$01&\no&\no&112 \\
82&J172220+6545.7&\no&33&\no&260.5844&65.7617&\no&\no&N&9.71e$-$01&8.34e$-$01&7.43e$-$01&\no&\no&103 \\
83&J172059+6545.1&\no&35&51&260.2470&65.7524&2.2517&\no&Q&4.02e$-$01&9.90e$-$01&7.19e$-$01&\no&\no&105 \\
84&J172433+6546.7&\no&36&412&261.1384&65.7796&\no&\no&N&6.94e$-$01&5.83e$-$01&5.18e$-$01&\no&\no&91 \\
85&J172302+6543.0&\no&37&\no&260.7593&65.7176&\no&\no&N&3.99e$-$01&8.77e$-$01&3.25e$-$01&\no&\no&135 \\
86&J172352+6542.9&\no&39&358&260.9668&65.7156&\no&0.32&N&5.40e$-$01&9.26e$-$01&7.46e$-$01&11.20& 0.82&171 \\
87&J172225+6542.1&\no&40&\no&260.6067&65.7017&\no&\no&N&6.80e$-$01&9.53e$-$01&6.32e$-$01&\no&\no&93 \\
88&J172140+6543.3&\no&41&\no&260.4205&65.7230&1.0811&\no&G&9.65e$-$01&9.33e$-$01&8.12e$-$01&\no&\no&105 \\
89&J172344+6543.4&\no&43&\no&260.9353&65.7238&\no&\no&N&7.18e$-$01&7.14e$-$01&8.68e$-$01&\no&\no&112 \\
90&J172000+6539.6&\no&44&\no&260.0025&65.6611&\no&\no&N&\no&\no&\no&\no&\no&48 \\
91&J172401+6538.4&\no&45&376&261.0064&65.6411&\no&\no&N&9.03e$-$01&7.14e$-$01&9.88e$-$01& 9.55&$-$0.19&170 \\
92&J172213+6538.2&\no&46&\no&260.5561&65.6374&\no&\no&N&2.44e$-$01&2.71e$-$01&3.33e$-$02&\no&\no&50 \\
93&J172423+6605.4&\no&47&\no&261.0959&66.0910&\no&\no&N&7.22e$-$01&3.69e$-$01&5.14e$-$01&\no&\no&58 \\
94&J172338+6603.4&\no&48&\no&260.9089&66.0577&\no&\no&N&7.32e$-$01&6.15e$-$01&2.38e$-$01&\no&\no&72 \\
95&J172048+6559.8&\no&49&\no&260.2038&65.9974&\no&\no&N&1.97e$-$02&5.92e$-$01&5.43e$-$02&\no&\no&286 \\
96&J172433+6556.0&\no&50&\no&261.1399&65.9339&\no&\no&N&1.62e$-$01&8.35e$-$01&3.38e$-$01&\no&\no&107 \\
97&J172351+6553.8&\no&51&\no&260.9640&65.8979&\no&\no&N&5.12e$-$01&9.03e$-$01&6.77e$-$01&\no&\no&127 \\
98&J172208+6555.0&\no&52&164&260.5340&65.9173&\no&\no&N&3.41e$-$01&9.85e$-$01&1.67e$-$01&\no&\no&115 \\
99&J172032+6553.5&\no&53&10&260.1348&65.8919&1.4216&\no&Q&9.07e$-$01&9.76e$-$01&7.60e$-$01&11.20& 1.25&131 \\
100&J172023+6545.8&\no&57&6&260.0987&65.7634&\no&\no&N&5.00e$-$01&1.04e$-$01&8.53e$-$02&\no&\no&183 \\
101&J172404+6545.3&\no&58&\no&261.0168&65.7558&\no&\no&N&8.55e$-$01&9.84e$-$01&9.43e$-$01&\no&\no&91 \\
102&J172401+6542.2&\no&60&372&261.0050&65.7046&1.6954&\no&Q&8.36e$-$01&9.24e$-$01&7.72e$-$01&10.70& 0.70&67 \\
103&J172108+6544.0&\no&61&68&260.2857&65.7342&1.1250&\no&Q&8.59e$-$01&9.16e$-$01&9.40e$-$01&10.09& 1.45&149 \\
104&J172446+6542.0&\no&62&425&261.1925&65.7010&\no&\no&N&3.60e$-$01&7.78e$-$01&2.14e$-$01&11.27& 0.42&96 \\
105&J172301+6541.4&\no&63&270&260.7545&65.6916&2.1507&\no&Q&8.18e$-$01&9.66e$-$01&9.02e$-$01&11.87& 1.14&64 \\
106&J172454+6543.3&\no&64&433&261.2276&65.7221&\no&0.39&N&7.57e$-$01&9.22e$-$01&9.95e$-$01&11.25& 2.33&151 \\
107&J172103+6540.8&\no&65&55&260.2654&65.6801&\no&\no&N&7.03e$-$01&8.73e$-$01&8.74e$-$01&11.96& 3.01&118 \\
108&J172432+6540.0&\no&66&413&261.1341&65.6676&\no&\no&N&4.29e$-$02&6.50e$-$01&5.75e$-$02&\no&\no&77 \\
109&J172046+6538.1&\no&67&31&260.1953&65.6361&\no&\no&N&6.15e$-$01&3.41e$-$01&3.78e$-$01&11.63& 1.26&54 \\
110&J172353+6603.1&\no&70&361&260.9728&66.0522&0.7831&\no&Q&4.15e$-$01&1.73e$-$01&1.57e$-$01& 8.94& 0.63&279 \\
111&J172327+6547.4&\no&73&317&260.8638&65.7900&1.7767&\no&Q&7.14e$-$01&6.50e$-$01&3.09e$-$01&11.60& 1.34&235 \\
112&J172250+6546.5&\no&74&233&260.7091&65.7763&\no&\no&N&9.93e$-$01&7.87e$-$01&7.96e$-$01&10.36& 0.69&112 \\


==> xmm_catalog.tex <==
1&275&\no&J172005+6556.2&\no&260.02274&65.93719&\no&\no&N&\no&\no&34 \\
2&283&\no&J172019+6550.4&\no&260.08170&65.84031&\no&\no&N&2.20e$-$01&1.00e+00&21 \\
3&\no&193&J172020+6546.2&\no&260.08680&65.77039&\no&\no&N&\no&\no&33 \\
4&236&\no&J172021+6549.3&\no&260.09048&65.82209&\no&\no&N&\no&\no&50 \\
5&262&\no&J172021+6556.9&\no&260.09131&65.94845&\no&\no&N&4.61e$-$01&2.76e$-$01&37 \\
6&\no&57&J172023+6545.5&100&260.09900&65.75884&\no&\no&N&\no&\no&46 \\
7&\no&202&J172026+6548.2&\no&260.10871&65.80489&\no&\no&N&1.00e+00&6.42e$-$02&41 \\
8&254&\no&J172027+6555.3&\no&260.11308&65.92297&\no&\no&N&4.28e$-$01&1.00e+00&23 \\
9&264&\no&J172027+6559.7&\no&260.11441&65.99651&\no&\no&N&6.34e$-$01&3.07e$-$01&43 \\
10&52&69&J172032+6553.3&99&260.13590&65.88961&1.4216&\no&Q&1.19e$-$01&7.69e$-$01&240 \\
11&\no&66&J172032+6545.2&\no&260.13724&65.75434&\no&\no&N&\no&\no&124 \\
12&281&\no&J172033+6558.7&\no&260.14013&65.97860&\no&\no&N&5.39e$-$01&9.24e$-$01&50 \\
13&\no&270&J172033+6539.2&\no&260.14122&65.65412&\no&\no&N&\no&\no&15 \\
14&93&\no&J172034+6554.6&\no&260.14496&65.91116&\no&\no&N&9.95e$-$01&6.39e$-$01&43 \\
15&\no&84&J172035+6540.5&\no&260.14623&65.67591&\no&\no&N&\no&\no&32 \\
16&\no&162&J172036+6552.2&\no&260.15211&65.87007&\no&\no&N&1.00e+00&8.43e$-$01&47 \\
17&\no&85&J172037+6537.4&\no&260.15454&65.62342&\no&\no&N&\no&\no&18 \\
18&\no&131&J172038+6541.0&\no&260.15997&65.68362&\no&\no&N&\no&\no&20 \\
19&188&\no&J172039+6547.7&\no&260.16260&65.79579&\no&\no&N&2.84e$-$01&1.00e+00&36 \\
20&\no&266&J172039+6549.9&\no&260.16387&65.83187&\no&\no&N&9.98e$-$01&6.09e$-$01&58 \\
21&235&\no&J172039+6601.7&\no&260.16625&66.02877&\no&\no&N&\no&\no&38 \\
22&234&\no&J172040+6601.1&\no&260.17043&66.01848&\no&\no&N&4.06e$-$01&6.88e$-$01&43 \\
23&194&\no&J172041+6558.1&\no&260.17155&65.96866&2.1878&\no&Q&6.54e$-$01&7.55e$-$01&77 \\
24&\no&221&J172041+6541.8&\no&260.17251&65.69671&\no&\no&N&\no&\no&30 \\
25&209&250&J172041+6546.4&\no&260.17271&65.77426&0.1715&\no&G&8.88e$-$01&9.39e$-$01&73 \\
26&\no&216&J172041+6539.8&\no&260.17330&65.66393&\no&\no&N&\no&\no&31 \\
27&103&\no&J172041+6555.6&\no&260.17456&65.92773&\no&\no&S&1.55e$-$01&1.00e+00&36 \\
28&\no&200&J172042+6544.0&\no&260.17535&65.73350&\no&\no&N&7.59e$-$01&6.76e$-$01&28 \\
29&176&\no&J172042+6557.0&\no&260.17866&65.95004&\no&\no&N&8.60e$-$01&7.27e$-$01&74 \\
30&120&\no&J172043+6553.3&\no&260.18232&65.88905&\no&\no&N&5.22e$-$01&9.64e$-$01&53 \\
31&\no&273&J172046+6538.2&109&260.19577&65.63765&\no&\no&N&\no&\no&58 \\
32&\no&249&J172047+6550.3&\no&260.19677&65.83887&\no&\no&N&9.42e$-$01&9.63e$-$01&54 \\
33&\no&237&J172047+6549.4&\no&260.19705&65.82444&\no&\no&N&9.99e$-$01&5.59e$-$01&51 \\
34&257&\no&J172047+6545.8&\no&260.19925&65.76395&\no&\no&N&1.00e+00&7.68e$-$01&42 \\
35&15&\no&J172048+6559.8&\no&260.20308&65.99749&0.4166&\no&G&3.73e$-$03&3.93e$-$01&351 \\
36&98&\no&J172049+6552.0&\no&260.20494&65.86735&\no&\no&N&7.80e$-$01&8.33e$-$01&76 \\
37&104&\no&J172052+6600.5&\no&260.21781&66.00882&0.4965&\no&G&9.62e$-$01&5.55e$-$01&85 \\
38&\no&174&J172052+6538.0&\no&260.21829&65.63360&\no&\no&N&\no&\no&25 \\
39&80&\no&J172053+6558.5&\no&260.22118&65.97569&1.6178&\no&Q&3.73e$-$01&7.45e$-$01&127 \\
40&160&\no&J172053+6554.8&\no&260.22325&65.91438&\no&\no&N&9.28e$-$01&8.29e$-$01&63 \\
41&\no&97&J172053+6544.1&\no&260.22340&65.73513&\no&\no&N&7.99e$-$01&5.86e$-$01&32 \\
42&44&261&J172053+6549.6&\no&260.22410&65.82769&\no&\no&S&2.65e$-$01&1.00e+00&184 \\
43&\no&248&J172053+6543.8&\no&260.22445&65.73118&\no&\no&N&4.43e$-$01&7.13e$-$01&46 \\
44&144&70&J172054+6552.8&\no&260.22682&65.88161&0.0040&\no&G&9.90e$-$01&9.99e$-$01&175 \\
45&251&\no&J172055+6548.3&\no&260.23306&65.80566&\no&\no&N&6.44e$-$01&9.99e$-$01&36 \\
46&263&\no&J172057+6600.0&\no&260.23780&66.00019&\no&\no&N&9.45e$-$01&2.33e$-$01&62 \\
47&258&\no&J172057+6549.2&\no&260.23803&65.82065&\no&\no&N&9.80e$-$01&9.82e$-$01&51 \\
48&\no&110&J172057+6549.0&\no&260.23914&65.81689&\no&\no&N&9.94e$-$01&6.79e$-$01&61 \\
49&140&78&J172058+6545.5&\no&260.24487&65.75975&\no&\no&N&9.86e$-$01&9.72e$-$01&177 \\
50&\no&102&J172058+6552.9&\no&260.24516&65.88195&\no&\no&N&9.98e$-$01&3.54e$-$01&69 \\
51&43&37&J172059+6544.9&83&260.24731&65.74912&2.2517&\no&Q&4.01e$-$01&8.28e$-$01&476 \\
52&102&72&J172100+6551.6&\no&260.25231&65.86155&0.7312&\no&Q&7.06e$-$01&9.11e$-$01&265 \\
53&\no&107&J172102+6544.3&\no&260.25834&65.73932&\no&\no&N&5.95e$-$01&9.65e$-$01&42 \\
54&\no&145&J172102+6552.8&\no&260.26024&65.88010&\no&\no&N&9.51e$-$01&8.24e$-$01&78 \\
55&\no&63&J172102+6540.7&107&260.26033&65.67935&\no&\no&N&6.00e$-$01&4.19e$-$01&241 \\
56&276&\no&J172102+6603.4&\no&260.26059&66.05764&\no&\no&N&\no&\no&39 \\
57&196&\no&J172102+6557.1&\no&260.26182&65.95219&\no&\no&N&9.38e$-$01&5.73e$-$01&63 \\
58&217&\no&J172103+6552.3&\no&260.26666&65.87277&\no&\no&N&9.98e$-$01&8.06e$-$01&51 \\
59&\no&244&J172104+6542.5&\no&260.26754&65.70956&\no&0.34&N&5.78e$-$01&9.37e$-$01&34 \\
60&\no&217&J172104+6538.6&\no&260.26756&65.64465&\no&\no&N&4.27e$-$01&\no&31 \\
61&\no&259&J172105+6537.0&\no&260.27231&65.61796&\no&\no&N&\no&\no&23 \\
62&152&\no&J172105+6554.4&\no&260.27358&65.90684&\no&\no&N&9.98e$-$01&5.69e$-$01&49 \\
63&\no&51&J172106+6548.0&\no&260.27812&65.80048&\no&\no&N&7.74e$-$01&9.99e$-$01&46 \\
64&\no&211&J172108+6555.2&\no&260.28361&65.92151&\no&0.39&N&9.13e$-$01&6.48e$-$01&60 \\
65&157&\no&J172108+6602.4&\no&260.28504&66.04101&\no&\no&N&5.25e$-$01&7.55e$-$01&104 \\
66&\no&94&J172108+6547.1&\no&260.28615&65.78602&\no&0.35&N&9.66e$-$01&9.01e$-$01&45 \\
67&200&\no&J172109+6602.0&\no&260.28769&66.03385&0.2712&\no&G&6.84e$-$01&7.93e$-$02&81 \\
68&16&17&J172109+6544.0&103&260.29119&65.73348&1.1250&\no&Q&7.91e$-$02&6.19e$-$01&957 \\
69&\no&179&J172110+6537.0&\no&260.29224&65.61752&\no&\no&N&\no&\no&20 \\
70&119&\no&J172110+6556.3&\no&260.29253&65.93937&\no&\no&N&6.40e$-$01&9.65e$-$01&107 \\
71&\no&239&J172110+6556.4&\no&260.29421&65.94120&\no&\no&Q&6.22e$-$01&9.23e$-$01&76 \\
72&223&\no&J172111+6548.5&\no&260.29599&65.80949&\no&\no&N&9.80e$-$01&9.99e$-$01&50 \\
73&123&\no&J172113+6554.4&\no&260.30509&65.90814&\no&\no&N&9.27e$-$01&9.77e$-$01&45 \\
74&105&133&J172113+6548.1&\no&260.30515&65.80202&0.7037&\no&G&7.91e$-$01&9.76e$-$01&167 \\
75&\no&177&J172116+6540.9&\no&260.32080&65.68167&\no&\no&N&5.60e$-$01&8.02e$-$01&92 \\
76&106&126&J172117+6545.2&\no&260.32093&65.75434&\no&\no&N&4.02e$-$01&9.45e$-$01&129 \\
77&246&\no&J172117+6544.6&\no&260.32370&65.74385&\no&\no&N&8.90e$-$01&9.26e$-$01&53 \\
78&170&\no&J172118+6602.2&\no&260.32833&66.03812&\no&\no&N&4.83e$-$01&4.83e$-$01&102 \\
79&78&182&J172118+6547.5&\no&260.32849&65.79276&0.3749&\no&G&6.64e$-$01&9.32e$-$01&245 \\
80&185&\no&J172118+6541.5&\no&260.32903&65.69266&\no&\no&N&9.17e$-$01&8.26e$-$01&25 \\
81&132&16&J172118+6545.8&\no&260.32911&65.76384&0.0090&\no&G&9.92e$-$01&9.32e$-$01&106 \\
82&\no&183&J172119+6544.1&\no&260.33031&65.73633&\no&\no&N&1.00e+00&9.73e$-$01&39 \\
83&145&251&J172119+6549.1&\no&260.33187&65.81939&\no&\no&N&4.26e$-$01&9.70e$-$01&117 \\
84&\no&105&J172119+6548.0&\no&260.33195&65.80134&\no&\no&N&7.57e$-$01&7.77e$-$01&102 \\
85&207&\no&J172119+6547.8&\no&260.33304&65.79742&\no&\no&N&6.64e$-$01&9.93e$-$01&34 \\
86&182&\no&J172120+6556.1&\no&260.33527&65.93622&0.0030&\no&G&6.14e$-$01&9.47e$-$01&60 \\
87&211&\no&J172120+6557.9&\no&260.33737&65.96513&\no&\no&N&6.16e$-$01&9.79e$-$01&40 \\
88&\no&165&J172121+6547.6&\no&260.33874&65.79390&\no&0.47&N&9.23e$-$01&9.53e$-$01&82 \\
89&\no&34&J172122+6537.7&\no&260.34464&65.62873&\no&\no&N&3.60e$-$03&3.13e$-$01&205 \\
90&268&\no&J172123+6557.3&\no&260.34622&65.95562&\no&\no&N&9.08e$-$01&9.13e$-$01&57 \\
91&\no&153&J172125+6547.6&\no&260.35774&65.79351&\no&\no&N&8.76e$-$01&8.61e$-$01&46 \\
92&\no&155&J172127+6545.3&\no&260.36330&65.75548&\no&\no&N&9.92e$-$01&7.80e$-$01&42 \\
93&\no&277&J172127+6548.0&\no&260.36362&65.80051&\no&\no&N&8.36e$-$01&9.99e$-$01&40 \\
94&284&\no&J172128+6548.4&\no&260.36923&65.80692&\no&\no&N&9.79e$-$01&9.60e$-$01&36 \\
95&50&98&J172129+6553.8&\no&260.37108&65.89732&\no&\no&N&9.34e$-$01&1.67e$-$01&292 \\
96&241&\no&J172129+6605.4&\no&260.37303&66.09088&\no&\no&N&\no&\no&45 \\
97&148&\no&J172130+6559.3&\no&260.37546&65.98937&\no&\no&N&9.75e$-$01&4.33e$-$01&40 \\
98&\no&269&J172130+6535.0&\no&260.37744&65.58356&\no&\no&N&\no&\no&22 \\
99&163&\no&J172132+6558.4&\no&260.38713&65.97468&\no&\no&N&9.70e$-$01&9.95e$-$01&57 \\
100&247&\no&J172136+6601.8&\no&260.40166&66.03059&\no&\no&N&7.65e$-$01&2.43e$-$01&59 \\
101&278&\no&J172136+6553.7&\no&260.40182&65.89567&\no&\no&N&1.00e+00&6.55e$-$01&37 \\
102&\no&149&J172136+6557.4&\no&260.40383&65.95687&\no&\no&N&1.00e+00&9.00e$-$01&67 \\
103&\no&228&J172137+6546.9&\no&260.40532&65.78197&\no&\no&N&9.90e$-$01&8.27e$-$01&46 \\
104&82&\no&J172137+6545.1&\no&260.40652&65.75288&\no&\no&N&5.51e$-$01&7.56e$-$01&68 \\
105&94&\no&J172139+6605.8&\no&260.41409&66.09740&1.6547&\no&Q&2.98e$-$01&6.88e$-$01&107 \\
106&231&\no&J172140+6554.4&\no&260.41968&65.90821&\no&\no&N&9.92e$-$01&5.86e$-$01&35 \\
107&272&\no&J172141+6556.9&\no&260.42296&65.94982&\no&\no&N&1.00e+00&8.60e$-$01&44 \\
108&3&7&J172142+6555.2&7&260.42658&65.92039&0.5233&\no&Q&7.05e$-$03&9.28e$-$01&1994 \\
109&118&\no&J172143+6554.2&\no&260.43048&65.90494&\no&\no&N&8.23e$-$01&4.61e$-$01&70 \\
110&\no&73&J172143+6543.1&\no&260.43141&65.71939&\no&\no&G&8.66e$-$01&9.73e$-$01&96 \\
111&2&5&J172143+6546.0&21&260.43200&65.76756&0.7813&\no&Q&1.70e$-$13&4.87e$-$02&3252 \\
112&45&180&J172143+6600.6&\no&260.43208&66.01057&\no&\no&N&1.43e$-$01&7.37e$-$01&172 \\
113&101&\no&J172144+6543.1&\no&260.43550&65.71912&0.9777&\no&G&5.72e$-$01&9.84e$-$01&66 \\
114&\no&187&J172144+6558.0&\no&260.43646&65.96769&\no&\no&N&8.58e$-$01&9.57e$-$01&125 \\
115&46&\no&J172145+6558.1&\no&260.43904&65.96955&1.4308&\no&Q&6.41e$-$01&9.48e$-$01&122 \\
116&\no&223&J172145+6558.2&\no&260.44091&65.97079&\no&\no&N&5.05e$-$01&7.50e$-$01&50 \\
117&166&\no&J172145+6548.6&\no&260.44163&65.81023&0.0023&\no&G&9.93e$-$01&9.88e$-$01&42 \\
118&\no&135&J172146+6551.8&\no&260.44484&65.86431&\no&\no&N&1.00e+00&9.62e$-$01&43 \\
119&243&\no&J172147+6558.7&\no&260.44824&65.97950&\no&\no&N&1.00e+00&7.83e$-$01&47 \\
120&\no&263&J172147+6541.6&\no&260.44856&65.69375&\no&0.54&N&7.53e$-$01&9.97e$-$01&61 \\
121&\no&36&J172147+6604.8&\no&260.44974&66.08036&\no&\no&N&5.44e$-$02&7.60e$-$01&146 \\
122&73&\no&J172148+6550.2&10&260.45078&65.83791&\no&\no&N&9.64e$-$01&3.88e$-$01&73 \\
123&\no&117&J172148+6545.6&\no&260.45224&65.76108&\no&\no&N&9.48e$-$01&7.52e$-$01&35 \\
124&\no&156&J172148+6551.4&\no&260.45270&65.85749&\no&\no&N&3.99e$-$01&9.64e$-$01&39 \\
125&135&61&J172148+6601.2&\no&260.45272&66.02130&0.1400&\no&G&9.32e$-$01&5.60e$-$01&122 \\
126&\no&14&J172149+6550.3&\no&260.45460&65.83862&\no&\no&N&6.96e$-$01&8.69e$-$01&48 \\
127&139&53&J172149+6559.8&70&260.45648&65.99708&\no&\no&N&9.99e$-$01&1.70e$-$01&204 \\
128&228&\no&J172150+6556.4&\no&260.45851&65.94002&\no&\no&N&9.99e$-$01&5.06e$-$01&32 \\
129&26&67&J172151+6552.5&34&260.46257&65.87610&\no&\no&N&2.84e$-$02&2.66e$-$01&288 \\
130&178&\no&J172151+6600.5&\no&260.46456&66.00947&\no&\no&N&7.31e$-$01&9.17e$-$01&62 \\
131&6&86&J172151+6604.8&\no&260.46602&66.08039&0.9130&\no&Q&6.52e$-$01&4.65e$-$01&1074 \\
132&216&\no&J172152+6545.8&\no&260.46780&65.76336&\no&\no&N&9.02e$-$01&1.00e+00&43 \\
133&74&\no&J172153+6603.3&\no&260.47143&66.05614&\no&\no&N&5.03e$-$01&5.19e$-$01&85 \\
134&34&203&J172153+6555.8&29&260.47189&65.93164&0.2699&\no&G&2.41e$-$01&8.93e$-$01&384 \\
135&85&\no&J172153+6541.0&\no&260.47344&65.68403&\no&\no&S&1.35e$-$01&9.99e$-$01&81 \\
136&\no&125&J172153+6556.1&\no&260.47421&65.93661&\no&\no&N&7.46e$-$01&7.21e$-$01&51 \\
137&40&52&J172155+6544.3&\no&260.48163&65.73922&\no&\no&N&4.46e$-$01&8.61e$-$01&300 \\
138&267&\no&J172156+6605.8&\no&260.48406&66.09750&\no&\no&N&1.00e+00&8.18e$-$01&46 \\
139&165&\no&J172156+6554.5&40&260.48524&65.90842&\no&\no&N&4.40e$-$01&9.62e$-$01&64 \\
140&\no&96&J172156+6559.4&\no&260.48601&65.99061&\no&\no&N&9.74e$-$01&9.85e$-$01&36 \\
141&131&\no&J172157+6555.2&\no&260.48805&65.92002&0.2800&\no&G&8.74e$-$01&9.91e$-$01&49 \\
142&\no&233&J172158+6544.1&22&260.49370&65.73568&\no&\no&N&8.93e$-$01&9.45e$-$01&37 \\
143&33&46&J172159+6550.3&\no&260.49688&65.83949&\no&\no&N&4.68e$-$01&8.08e$-$01&364 \\
144&112&124&J172159+6554.5&40&260.49850&65.90995&\no&\no&G&4.66e$-$01&9.10e$-$01&205 \\
145&71&246&J172159+6550.0&\no&260.49972&65.83346&\no&\no&G&3.12e$-$01&9.92e$-$01&190 \\
146&206&\no&J172201+6602.5&\no&260.50424&66.04201&\no&\no&N&1.00e+00&3.04e$-$01&37 \\
147&221&118&J172201+6546.1&\no&260.50571&65.76848&\no&\no&N&5.95e$-$01&8.75e$-$01&131 \\
148&28&38&J172201+6544.0&22&260.50734&65.73407&\no&\no&G&4.07e$-$02&6.87e$-$01&521 \\
149&173&\no&J172203+6547.2&\no&260.51603&65.78767&\no&\no&N&1.00e+00&8.95e$-$01&39 \\
150&113&\no&J172204+6601.2&\no&260.51874&66.02086&\no&\no&N&9.73e$-$01&4.41e$-$01&63 \\
151&\no&129&J172204+6604.1&\no&260.52001&66.06879&\no&\no&N&8.27e$-$01&2.97e$-$01&42 \\
152&\no&178&J172205+6555.1&\no&260.52415&65.91893&\no&\no&N&9.00e$-$01&9.99e$-$01&52 \\
153&72&\no&J172205+6604.1&\no&260.52422&66.06981&\no&\no&N&9.84e$-$01&5.41e$-$01&115 \\
154&37&47&J172205+6557.2&28&260.52446&65.95491&\no&\no&N&6.19e$-$01&8.86e$-$01&354 \\
155&\no&175&J172206+6555.4&\no&260.52758&65.92450&\no&0.39&N&3.76e$-$01&9.97e$-$01&120 \\
156&90&\no&J172207+6555.3&\no&260.52934&65.92272&\no&\no&N&2.97e$-$01&9.19e$-$01&70 \\
157&\no&185&J172208+6535.1&\no&260.53342&65.58542&\no&\no&N&6.42e$-$01&9.82e$-$02&31 \\
158&273&\no&J172208+6551.3&\no&260.53407&65.85633&\no&\no&N&9.93e$-$01&7.67e$-$01&30 \\
159&213&\no&J172208+6559.3&\no&260.53452&65.98851&\no&\no&N&9.07e$-$01&9.63e$-$01&50 \\
160&\no&103&J172208+6545.2&12&260.53572&65.75480&\no&\no&N&9.97e$-$01&9.66e$-$01&47 \\
161&117&82&J172208+6557.0&71&260.53648&65.95028&\no&\no&N&9.69e$-$01&2.47e$-$01&268 \\
162&62&234&J172208+6553.6&\no&260.53665&65.89417&\no&\no&N&8.09e$-$01&9.05e$-$01&166 \\
163&56&68&J172208+6547.7&36&260.53710&65.79518&2.2508&\no&Q&2.05e$-$01&9.59e$-$01&352 \\
164&18&32&J172208+6554.9&98&260.53720&65.91661&\no&\no&N&5.40e$-$01&5.80e$-$01&538 \\
165&\no&90&J172209+6549.6&\no&260.53848&65.82712&\no&1.24&N&9.99e$-$01&7.27e$-$01&40 \\
166&177&83&J172209+6541.0&\no&260.54108&65.68467&1.9072&\no&Q&1.23e$-$01&7.06e$-$01&193 \\
167&219&\no&J172210+6545.1&\no&260.54255&65.75193&\no&\no&N&9.25e$-$01&9.94e$-$01&45 \\
168&\no&208&J172210+6536.1&\no&260.54459&65.60302&\no&\no&N&3.66e$-$01&9.88e$-$01&54 \\
169&\no&10&J172211+6545.0&\no&260.54650&65.75141&\no&\no&N&9.73e$-$01&9.83e$-$01&44 \\
170&181&\no&J172211+6556.5&56&260.54947&65.94302&\no&\no&N&1.00e+00&8.39e$-$01&46 \\
171&162&\no&J172211+6555.6&\no&260.54956&65.92747&0.5832&\no&G&9.16e$-$01&9.50e$-$01&64 \\
172&240&\no&J172211+6553.2&32&260.54995&65.88802&\no&\no&N&9.82e$-$01&4.57e$-$01&32 \\
173&232&\no&J172212+6548.7&\no&260.55195&65.81329&\no&\no&N&9.12e$-$01&9.98e$-$01&39 \\
174&27&\no&J172212+6601.6&\no&260.55228&66.02718&0.4968&\no&Q&3.10e$-$01&4.33e$-$01&159 \\
175&\no&240&J172212+6555.5&\no&260.55296&65.92528&\no&\no&N&8.77e$-$01&9.98e$-$01&65 \\
176&242&\no&J172212+6601.0&\no&260.55305&66.01764&0.5886&\no&G&5.51e$-$01&9.11e$-$01&50 \\
177&190&\no&J172212+6538.8&\no&260.55380&65.64800&\no&\no&N&9.94e$-$01&7.35e$-$01&44 \\
178&261&\no&J172213+6555.4&\no&260.55572&65.92406&\no&\no&N&8.92e$-$01&1.00e+00&36 \\
179&\no&151&J172213+6601.0&\no&260.55678&66.01717&\no&0.48&N&5.36e$-$01&3.57e$-$01&90 \\
180&230&\no&J172213+6554.4&\no&260.55687&65.90754&\no&\no&N&9.29e$-$01&9.35e$-$01&34 \\
181&122&\no&J172215+6604.0&\no&260.56469&66.06693&\no&\no&N&7.76e$-$01&7.42e$-$01&106 \\
182&191&\no&J172215+6553.5&\no&260.56543&65.89332&\no&\no&N&1.00e+00&6.98e$-$01&31 \\
183&134&\no&J172216+6557.1&56&260.56864&65.95296&\no&0.47&N&8.64e$-$01&9.52e$-$01&67 \\
184&77&77&J172217+6538.5&\no&260.57141&65.64297&\no&\no&N&2.90e$-$01&4.00e$-$01&169 \\
185&\no&101&J172217+6540.1&\no&260.57209&65.66883&\no&\no&N&9.99e$-$01&8.66e$-$01&39 \\
186&\no&278&J172217+6541.6&\no&260.57354&65.69425&\no&\no&N&1.00e+00&8.60e$-$01&34 \\
187&218&\no&J172217+6552.6&\no&260.57431&65.87692&0.5989&\no&G&9.54e$-$01&9.58e$-$01&46 \\
188&83&245&J172217+6600.0&\no&260.57447&66.00075&\no&\no&N&4.50e$-$01&9.46e$-$01&128 \\
189&22&88&J172218+6600.5&\no&260.57632&66.00975&0.4966&\no&Q&7.50e$-$01&7.90e$-$01&481 \\
190&158&\no&J172218+6539.0&\no&260.57826&65.65064&\no&\no&N&1.00e+00&6.03e$-$01&39 \\
191&256&\no&J172218+6553.6&\no&260.57840&65.89459&0.2200&\no&G&9.95e$-$01&7.96e$-$01&40 \\
192&108&134&J172218+6546.0&\no&260.57875&65.76796&\no&\no&G&5.99e$-$01&7.36e$-$01&116 \\
193&66&49&J172219+6544.2&13&260.58053&65.73792&1.0190&\no&Q&3.19e$-$02&5.62e$-$01&318 \\
194&21&81&J172220+6545.2&\no&260.58385&65.75477&\no&\no&N&2.37e$-$03&5.55e$-$01&497 \\
195&\no&143&J172221+6542.4&\no&260.59046&65.70669&\no&\no&N&9.04e$-$01&9.06e$-$01&49 \\
196&\no&231&J172223+6604.6&\no&260.59665&66.07719&\no&\no&N&5.23e$-$01&4.10e$-$01&32 \\
197&\no&227&J172223+6535.9&\no&260.59924&65.59835&\no&\no&N&1.00e+00&7.14e$-$01&29 \\
198&\no&254&J172224+6554.8&\no&260.60099&65.91423&\no&\no&N&9.75e$-$01&8.97e$-$01&46 \\
199&250&\no&J172224+6554.9&\no&260.60156&65.91579&\no&\no&N&7.90e$-$01&9.95e$-$01&49 \\
200&53&87&J172224+6545.4&\no&260.60350&65.75705&1.9486&\no&Q&6.26e$-$01&9.41e$-$01&219 \\
201&280&\no&J172225+6548.2&\no&260.60423&65.80356&\no&\no&N&9.81e$-$01&8.88e$-$01&58 \\
202&237&\no&J172225+6606.0&\no&260.60503&66.10123&\no&\no&N&8.01e$-$01&9.05e$-$01&63 \\
203&\no&242&J172226+6554.6&\no&260.60998&65.91156&\no&\no&N&1.00e+00&9.31e$-$01&49 \\
204&168&\no&J172227+6557.8&\no&260.61449&65.96432&\no&\no&N&3.09e$-$01&9.22e$-$01&53 \\
205&171&\no&J172229+6601.8&\no&260.62283&66.03087&0.5901&\no&G&9.90e$-$01&4.31e$-$01&35 \\
206&286&\no&J172229+6604.9&\no&260.62283&66.08322&\no&\no&N&9.94e$-$01&6.52e$-$01&60 \\
207&60&\no&J172229+6558.7&25&260.62403&65.97857&\no&\no&S&9.15e$-$01&6.64e$-$02&118 \\
208&97&115&J172229+6555.1&30&260.62427&65.91998&\no&\no&N&7.38e$-$01&8.07e$-$01&154 \\
209&23&114&J172231+6602.7&\no&260.63322&66.04645&0.1682&\no&G&1.33e$-$01&7.08e$-$01&285 \\
210&253&\no&J172232+6554.4&\no&260.63427&65.90680&\no&\no&N&9.98e$-$01&9.31e$-$01&46 \\
211&\no&138&J172232+6538.0&\no&260.63564&65.63376&\no&\no&N&7.08e$-$01&9.53e$-$01&38 \\
212&220&\no&J172232+6547.6&\no&260.63689&65.79417&\no&\no&N&8.61e$-$01&8.97e$-$01&47 \\
213&5&11&J172233+6550.6&16&260.63987&65.84489&1.3369&\no&Q&2.20e$-$03&1.28e$-$04&1796 \\
214&\no&113&J172235+6602.7&\no&260.64988&66.04536&\no&\no&N&9.94e$-$01&6.71e$-$01&55 \\
215&100&121&J172236+6552.2&\no&260.65013&65.87075&\no&\no&N&8.98e$-$01&7.57e$-$01&198 \\
216&\no&210&J172236+6555.8&\no&260.65165&65.93141&\no&\no&G&1.00e+00&6.95e$-$01&43 \\
217&238&\no&J172238+6604.2&\no&260.65844&66.07126&\no&\no&N&9.96e$-$01&6.48e$-$01&48 \\
218&47&31&J172238+6555.7&6&260.66056&65.92911&\no&\no&N&1.00e+00&1.10e$-$01&205 \\
219&\no&91&J172238+6549.6&\no&260.66187&65.82826&\no&\no&N&8.17e$-$01&9.25e$-$01&35 \\
220&121&169&J172239+6543.7&\no&260.66524&65.72908&\no&\no&N&3.13e$-$01&1.82e$-$01&207 \\
221&183&\no&J172240+6554.4&\no&260.66933&65.90773&\no&\no&N&9.35e$-$01&9.94e$-$01&62 \\
222&17&3&J172241+6542.6&23&260.67174&65.71137&0.1791&\no&G&9.97e$-$01&1.65e$-$09&1019 \\
223&39&\no&J172241+6604.6&\no&260.67246&66.07807&\no&\no&N&1.34e$-$01&8.57e$-$01&124 \\
224&197&\no&J172242+6546.1&\no&260.67806&65.76849&\no&\no&N&1.00e+00&7.00e$-$01&34 \\
225&214&\no&J172242+6550.0&\no&260.67910&65.83468&\no&\no&N&9.99e$-$01&6.01e$-$01&45 \\
226&114&194&J172245+6549.7&\no&260.68925&65.82940&0.4991&\no&G&8.64e$-$01&9.57e$-$01&150 \\
227&49&15&J172245+6544.2&3&260.69051&65.73788&\no&\no&N&6.04e$-$01&3.41e$-$01&342 \\
228&142&\no&J172246+6557.9&\no&260.69262&65.96649&\no&\no&N&7.98e$-$01&9.90e$-$01&36 \\
229&69&50&J172246+6548.3&44&260.69321&65.80515&\no&\no&N&1.27e$-$01&2.65e$-$01&253 \\
230&167&\no&J172246+6545.2&\no&260.69400&65.75349&\no&\no&N&9.82e$-$01&8.58e$-$01&52 \\
231&\no&206&J172246+6535.7&\no&260.69568&65.59641&\no&\no&N&7.37e$-$01&1.00e+00&33 \\
232&\no&238&J172247+6533.6&\no&260.69838&65.56115&\no&\no&N&\no&\no&34 \\
233&35&29&J172247+6546.6&112&260.69845&65.77779&\no&\no&N&6.32e$-$01&7.21e$-$01&406 \\
234&136&\no&J172248+6549.5&\no&260.70082&65.82546&0.4740&\no&G&7.66e$-$01&9.91e$-$01&40 \\
235&84&168&J172248+6548.7&\no&260.70237&65.81276&\no&\no&N&5.68e$-$01&7.61e$-$01&141 \\
236&260&\no&J172249+6553.9&\no&260.70477&65.89850&\no&\no&N&9.59e$-$01&8.72e$-$01&34 \\
237&193&21&J172249+6553.4&76&260.70495&65.89071&0.0011&\no&G&7.70e$-$01&9.74e$-$01&123 \\
238&\no&76&J172249+6550.2&78&260.70814&65.83824&\no&1.46&N&9.93e$-$01&4.64e$-$01&55 \\
239&186&252&J172250+6557.7&\no&260.71163&65.96191&\no&\no&N&9.10e$-$01&9.99e$-$01&80 \\
240&147&\no&J172251+6558.2&\no&260.71323&65.97126&\no&\no&N&9.93e$-$01&6.99e$-$01&56 \\
241&99&60&J172251+6600.6&48&260.71529&66.01079&\no&\no&N&7.88e$-$01&9.59e$-$01&227 \\
242&107&24&J172251+6547.5&\no&260.71649&65.79297&\no&\no&N&6.08e$-$02&9.31e$-$01&300 \\
243&244&\no&J172252+6541.1&\no&260.71688&65.68580&\no&\no&N&9.25e$-$01&1.00e+00&54 \\
244&202&\no&J172252+6604.9&\no&260.71794&66.08178&\no&\no&N&6.20e$-$01&9.61e$-$01&49 \\
245&125&\no&J172252+6543.7&\no&260.71849&65.72888&\no&\no&N&2.90e$-$01&1.00e+00&50 \\
246&\no&75&J172253+6541.0&\no&260.72096&65.68452&\no&\no&Q&4.01e$-$01&6.33e$-$01&153 \\
247&138&\no&J172253+6553.5&33&260.72138&65.89284&\no&\no&N&8.43e$-$01&9.01e$-$01&67 \\
248&42&212&J172253+6541.9&60&260.72356&65.69895&\no&0.44&N&8.46e$-$01&7.76e$-$01&202 \\
249&\no&192&J172253+6539.2&\no&260.72393&65.65458&\no&\no&N&9.62e$-$01&9.37e$-$01&62 \\
250&282&\no&J172253+6554.8&\no&260.72401&65.91452&\no&\no&N&9.28e$-$01&7.01e$-$01&39 \\
251&110&275&J172253+6542.3&\no&260.72449&65.70624&\no&\no&S&6.29e$-$01&9.95e$-$01&180 \\
252&\no&80&J172254+6548.0&\no&260.72838&65.80121&\no&0.35&N&8.11e$-$01&9.71e$-$01&148 \\
253&201&\no&J172255+6547.9&\no&260.73029&65.79879&\no&\no&N&6.69e$-$01&9.93e$-$01&52 \\
254&32&39&J172255+6553.4&33&260.73196&65.89016&0.6007&\no&Q&8.19e$-$01&9.50e$-$01&382 \\
255&\no&116&J172255+6542.1&\no&260.73288&65.70232&\no&\no&N&9.48e$-$01&9.89e$-$01&112 \\
256&\no&184&J172256+6544.8&\no&260.73366&65.74779&\no&0.84&N&1.00e+00&6.39e$-$01&47 \\
257&\no&265&J172257+6541.0&\no&260.73832&65.68419&\no&\no&N&7.45e$-$01&9.41e$-$01&39 \\
258&133&\no&J172257+6542.1&\no&260.73857&65.70237&\no&\no&N&9.32e$-$01&9.45e$-$01&66 \\
259&115&\no&J172257+6542.4&\no&260.74009&65.70719&0.1582&\no&G&9.17e$-$01&8.95e$-$01&60 \\
260&203&\no&J172257+6554.3&15&260.74060&65.90585&\no&\no&N&9.43e$-$01&8.39e$-$01&48 \\
261&\no&139&J172258+6605.0&\no&260.74179&66.08402&\no&\no&N&3.25e$-$01&9.36e$-$01&24 \\
262&233&\no&J172258+6604.8&\no&260.74291&66.08048&0.2935&\no&G&7.34e$-$01&7.33e$-$01&78 \\
263&\no&161&J172258+6537.9&\no&260.74458&65.63216&\no&\no&N&7.03e$-$01&9.65e$-$01&126 \\
264&96&132&J172259+6558.7&\no&260.74669&65.97888&\no&\no&N&7.72e$-$01&8.75e$-$01&141 \\
265&\no&181&J172259+6547.5&\no&260.74911&65.79175&\no&1.06&N&2.44e$-$01&7.52e$-$01&193 \\
266&10&27&J172300+6554.6&15&260.75260&65.91031&\no&\no&N&6.61e$-$02&6.94e$-$01&649 \\
267&88&\no&J172301+6605.0&\no&260.75550&66.08405&\no&\no&N&7.23e$-$01&2.20e$-$01&102 \\
268&146&\no&J172301+6549.1&\no&260.75613&65.81857&0.0001&\no&G&3.11e$-$01&9.79e$-$01&86 \\
269&179&13&J172301+6548.0&\no&260.75788&65.80040&0.1792&\no&G&8.11e$-$01&9.78e$-$01&106 \\
270&24&74&J172302+6541.4&105&260.75950&65.69061&2.1507&\no&Q&2.22e$-$01&2.07e$-$01&307 \\
271&81&\no&J172303+6557.5&\no&260.76422&65.95892&\no&\no&N&7.39e$-$01&9.91e$-$01&83 \\
272&215&\no&J172303+6602.3&\no&260.76573&66.03839&\no&\no&N&9.67e$-$01&9.51e$-$01&58 \\
273&65&\no&J172304+6546.7&52&260.76844&65.77948&\no&\no&N&7.23e$-$01&7.58e$-$01&77 \\
274&87&\no&J172305+6547.5&\no&260.77125&65.79168&\no&\no&N&7.84e$-$01&7.57e$-$01&70 \\
275&\no&204&J172305+6602.1&\no&260.77397&66.03614&\no&\no&N&7.82e$-$01&8.83e$-$01&62 \\
276&\no&25&J172305+6603.5&\no&260.77421&66.05943&\no&0.32&N&8.36e$-$01&9.51e$-$01&46 \\
277&76&\no&J172306+6552.5&35&260.77505&65.87582&\no&\no&N&4.87e$-$01&9.88e$-$01&79 \\
278&\no&128&J172306+6548.7&\no&260.77586&65.81293&\no&1.81&N&9.35e$-$01&9.66e$-$01&49 \\
279&13&9&J172306+6551.3&19&260.77701&65.85518&0.8846&\no&Q&7.16e$-$01&1.60e$-$01&572 \\
280&198&\no&J172306+6602.0&\no&260.77843&66.03480&\no&\no&N&9.50e$-$01&7.57e$-$01&61 \\
281&54&45&J172306+6546.4&52&260.77880&65.77399&0.6339&\no&Q&3.45e$-$01&8.71e$-$01&420 \\
282&111&142&J172307+6557.0&\no&260.78103&65.95067&\no&\no&G&5.92e$-$01&4.78e$-$01&162 \\
283&\no&1&J172307+6547.8&\no&260.78170&65.79815&\no&\no&N&8.60e$-$01&7.85e$-$01&56 \\
284&\no&108&J172308+6603.5&\no&260.78532&66.05931&\no&\no&N&7.20e$-$01&9.96e$-$01&40 \\
285&68&170&J172308+6550.6&\no&260.78683&65.84394&\no&\no&N&9.36e$-$01&7.65e$-$01&126 \\
286&63&243&J172308+6552.5&35&260.78718&65.87606&\no&\no&N&8.54e$-$01&6.07e$-$01&234 \\
287&\no&89&J172309+6552.2&\no&260.78826&65.87163&\no&\no&N&9.17e$-$01&7.28e$-$01&108 \\
288&29&44&J172309+6548.1&\no&260.78848&65.80275&1.6000&\no&Q&6.97e$-$01&3.46e$-$01&388 \\
289&\no&93&J172309+6549.2&\no&260.79152&65.82082&\no&\no&N&9.23e$-$01&9.29e$-$01&82 \\
290&155&\no&J172311+6554.9&\no&260.79891&65.91508&\no&\no&N&9.82e$-$01&8.80e$-$01&51 \\
291&116&\no&J172312+6543.4&\no&260.80156&65.72481&\no&\no&N&9.66e$-$01&7.60e$-$01&68 \\
292&19&235&J172312+6603.5&\no&260.80286&66.05852&0.0139&\no&G&1.78e$-$02&6.49e$-$02&372 \\
293&67&\no&J172313+6553.0&\no&260.80642&65.88498&\no&\no&N&9.59e$-$01&7.75e$-$01&132 \\
294&130&\no&J172313+6555.3&\no&260.80678&65.92192&\no&\no&N&9.92e$-$01&9.02e$-$01&70 \\
295&\no&230&J172313+6540.3&\no&260.80679&65.67228&\no&\no&N&8.05e$-$01&9.99e$-$01&37 \\
296&\no&191&J172313+6553.1&\no&260.80814&65.88652&\no&\no&N&8.95e$-$01&8.19e$-$01&158 \\
297&149&\no&J172313+6541.7&\no&260.80818&65.69612&\no&\no&N&5.27e$-$01&1.00e+00&51 \\
298&\no&55&J172314+6546.0&\no&260.80852&65.76814&\no&\no&N&1.00e+00&4.68e$-$01&50 \\
299&1&2&J172314+6547.7&9&260.80910&65.79614&1.4411&\no&Q&8.05e$-$08&1.43e$-$03&10699 \\
300&175&253&J172314+6556.1&\no&260.81212&65.93585&\no&\no&N&8.64e$-$01&6.71e$-$01&102 \\
301&\no&157&J172315+6538.6&\no&260.81546&65.64334&\no&\no&N&6.17e$-$01&7.03e$-$01&46 \\
302&\no&229&J172316+6550.5&\no&260.81743&65.84227&\no&\no&N&7.92e$-$01&8.97e$-$01&55 \\
303&\no&226&J172316+6553.8&\no&260.81863&65.89779&\no&0.34&N&8.77e$-$01&8.81e$-$01&40 \\
304&274&\no&J172316+6550.4&\no&260.82073&65.84102&\no&\no&N&9.93e$-$01&9.96e$-$01&63 \\
305&12&8&J172317+6556.6&5&260.82413&65.94352&0.4949&\no&G&7.59e$-$05&6.69e$-$04&937 \\
306&\no&218&J172318+6553.3&\no&260.82556&65.88899&\no&\no&N&9.99e$-$01&9.41e$-$01&45 \\
307&195&\no&J172319+6557.9&\no&260.82957&65.96640&\no&\no&N&9.37e$-$01&9.81e$-$01&45 \\
308&\no&54&J172320+6539.7&\no&260.83410&65.66212&\no&\no&N&9.23e$-$01&8.99e$-$01&108 \\
309&\no&164&J172321+6536.2&\no&260.83776&65.60387&\no&0.13&N&7.44e$-$01&7.30e$-$01&31 \\
310&\no&109&J172322+6549.6&\no&260.84197&65.82805&\no&1.61&N&9.98e$-$01&9.34e$-$01&42 \\
311&128&\no&J172323+6601.2&\no&260.84780&66.02012&\no&\no&N&8.18e$-$01&9.23e$-$01&56 \\
312&59&190&J172323+6558.5&\no&260.84785&65.97537&\no&\no&N&6.61e$-$01&9.97e$-$01&151 \\
313&\no&271&J172323+6538.3&\no&260.84929&65.63964&\no&\no&N&9.48e$-$01&9.97e$-$01&37 \\
314&248&\no&J172325+6551.2&\no&260.85748&65.85428&\no&\no&N&7.48e$-$01&9.98e$-$01&65 \\
315&\no&215&J172326+6551.1&\no&260.85911&65.85282&\no&0.91&N&8.84e$-$01&9.94e$-$01&52 \\
316&\no&272&J172326+6538.2&\no&260.85982&65.63776&\no&\no&N&6.73e$-$01&9.42e$-$01&105 \\
317&8&28&J172326+6547.2&111&260.86125&65.78808&1.7855&\no&Q&7.40e$-$03&9.23e$-$01&864 \\
318&11&35&J172328+6559.2&4&260.86706&65.98726&1.4252&\no&Q&2.39e$-$04&4.41e$-$01&664 \\
319&225&\no&J172329+6552.1&\no&260.87153&65.86926&\no&\no&N&9.99e$-$01&9.11e$-$01&34 \\
320&70&95&J172329+6541.9&\no&260.87216&65.69922&2.7418&\no&Q&1.66e$-$01&4.24e$-$01&218 \\
321&124&41&J172329+6548.7&\no&260.87333&65.81302&\no&\no&N&6.61e$-$01&1.49e$-$01&215 \\
322&41&220&J172329+6553.8&\no&260.87462&65.89672&1.1226&\no&Q&2.39e$-$01&7.97e$-$01&203 \\
323&\no&256&J172329+6538.1&\no&260.87472&65.63573&\no&\no&N&9.73e$-$01&6.19e$-$01&34 \\
324&58&64&J172331+6601.6&\no&260.88120&66.02738&0.5898&\no&G&9.59e$-$02&7.48e$-$01&236 \\
325&169&104&J172333+6546.9&46&260.89100&65.78244&0.4031&\no&G&9.07e$-$01&7.58e$-$01&154 \\
326&239&\no&J172335+6600.3&\no&260.89618&66.00666&\no&\no&N&7.59e$-$01&9.94e$-$01&46 \\
327&14&22&J172335+6549.0&20&260.89721&65.81750&0.7791&\no&G&9.38e$-$04&9.91e$-$02&534 \\
328&269&\no&J172335+6543.0&\no&260.89731&65.71767&\no&\no&N&9.78e$-$01&7.09e$-$01&43 \\
329&\no&255&J172337+6539.0&\no&260.90618&65.65070&\no&\no&N&9.01e$-$13&9.93e$-$01&180 \\
330&229&\no&J172339+6548.4&\no&260.91285&65.80804&\no&\no&N&1.00e+00&3.88e$-$01&35 \\
331&109&247&J172339+6600.8&\no&260.91347&66.01473&\no&\no&N&4.50e$-$01&7.74e$-$01&119 \\
332&226&\no&J172340+6543.6&\no&260.91720&65.72682&\no&\no&N&8.13e$-$01&9.12e$-$01&39 \\
333&\no&205&J172341+6601.8&\no&260.92187&66.03063&\no&0.52&N&5.54e$-$01&6.82e$-$01&54 \\
334&\no&198&J172341+6539.1&\no&260.92291&65.65243&\no&\no&N&7.53e$-$01&1.00e+00&38 \\
335&89&141&J172341+6545.2&\no&260.92316&65.75393&\no&\no&G&2.84e$-$01&5.60e$-$01&183 \\
336&127&\no&J172341+6551.9&\no&260.92338&65.86644&\no&\no&N&6.10e$-$01&9.79e$-$01&59 \\
337&\no&122&J172341+6549.0&\no&260.92393&65.81829&\no&\no&N&9.98e$-$01&6.45e$-$01&44 \\
338&48&\no&J172342+6601.8&\no&260.92532&66.03053&\no&\no&N&7.32e$-$02&6.13e$-$01&97 \\
339&\no&33&J172342+6545.9&\no&260.92734&65.76557&\no&0.22&N&7.99e$-$01&9.68e$-$01&44 \\
340&184&\no&J172343+6541.5&\no&260.93024&65.69318&\no&\no&N&8.55e$-$01&9.93e$-$01&35 \\
341&31&257&J172343+6602.5&\no&260.93161&66.04227&\no&\no&N&4.00e$-$01&7.41e$-$01&134 \\
342&79&65&J172343+6540.5&\no&260.93185&65.67561&1.0544&\no&Q&4.70e$-$02&9.85e$-$01&294 \\
343&126&\no&J172343+6540.9&\no&260.93327&65.68298&\no&\no&N&3.26e$-$01&8.88e$-$01&40 \\
344&161&\no&J172344+6553.1&\no&260.93721&65.88617&\no&\no&N&6.15e$-$01&9.99e$-$01&50 \\
345&\no&166&J172345+6535.6&\no&260.94033&65.59483&\no&\no&N&2.34e$-$01&8.43e$-$01&59 \\
346&\no&6&J172347+6603.0&\no&260.94628&66.05078&\no&\no&N&9.64e$-$01&4.33e$-$01&106 \\
347&91&197&J172347+6554.4&\no&260.94769&65.90776&4.1150&\no&Q&5.24e$-$01&8.49e$-$01&266 \\
348&\no&213&J172349+6534.1&\no&260.95485&65.56848&\no&\no&N&\no&\no&32 \\
349&159&\no&J172349+6544.7&\no&260.95515&65.74518&0.5919&\no&G&9.12e$-$01&9.21e$-$01&54 \\
350&55&222&J172349+6551.7&\no&260.95665&65.86309&\no&\no&N&5.95e$-$01&9.78e$-$01&141 \\
351&137&\no&J172349+6554.4&\no&260.95697&65.90768&\no&\no&N&8.56e$-$01&9.53e$-$01&56 \\
352&25&30&J172349+6542.9&\no&260.95815&65.71590&\no&\no&N&7.75e$-$01&5.05e$-$01&568 \\
353&150&\no&J172349+6549.3&\no&260.95817&65.82235&\no&\no&N&9.96e$-$01&7.61e$-$01&36 \\
354&151&\no&J172350+6602.0&\no&260.96230&66.03481&\no&\no&N&9.48e$-$01&6.30e$-$01&68 \\
355&153&\no&J172350+6544.3&\no&260.96235&65.73834&\no&\no&N&9.95e$-$01&9.24e$-$01&59 \\
356&7&58&J172351+6550.0&43&260.96533&65.83485&0.6726&\no&Q&2.30e$-$08&2.72e$-$01&673 \\
357&75&79&J172351+6545.8&\no&260.96630&65.76379&\no&\no&N&8.42e$-$01&9.50e$-$01&227 \\
358&\no&120&J172352+6543.0&86&260.96794&65.71777&\no&0.32&N&8.16e$-$01&9.14e$-$01&42 \\
359&\no&111&J172352+6602.0&\no&260.96849&66.03440&\no&\no&N&4.44e$-$01&6.78e$-$01&52 \\
360&259&\no&J172352+6604.9&\no&260.97014&66.08219&\no&\no&N&\no&\no&39 \\
361&9&20&J172353+6603.0&110&260.97416&66.05023&0.7831&\no&Q&3.07e$-$03&6.01e$-$02&1069 \\
362&129&207&J172354+6603.4&\no&260.97601&66.05711&\no&\no&N&5.90e$-$01&8.08e$-$01&97 \\
363&\no&42&J172354+6534.3&\no&260.97660&65.57261&\no&0.48&N&\no&\no&184 \\
364&\no&4&J172355+6600.5&\no&260.97965&66.00968&\no&\no&G&9.98e$-$01&9.72e$-$01&107 \\
365&143&172&J172355+6542.7&\no&260.98179&65.71216&\no&\no&G&9.53e$-$01&9.08e$-$01&160 \\
366&\no&140&J172356+6538.6&\no&260.98563&65.64473&\no&\no&N&9.46e$-$01&5.68e$-$01&39 \\
367&141&40&J172356+6549.4&17&260.98668&65.82446&\no&\no&N&4.88e$-$01&9.09e$-$01&180 \\
368&\no&106&J172358+6549.1&\no&260.99231&65.81963&\no&\no&N&1.00e+00&7.71e$-$01&44 \\
369&212&\no&J172358+6601.9&\no&260.99268&66.03250&\no&\no&N&9.38e$-$01&7.84e$-$01&72 \\
370&\no&130&J172358+6538.9&\no&260.99315&65.64845&\no&\no&N&1.90e$-$01&5.11e$-$01&159 \\
371&270&\no&J172400+6604.9&\no&261.00007&66.08312&0.2712&\no&G&\no&\no&45 \\
372&38&23&J172400+6542.1&102&261.00113&65.70211&1.6954&\no&Q&7.75e$-$02&7.12e$-$01&802 \\
373&30&48&J172400+6557.6&\no&261.00265&65.96073&1.1927&\no&Q&3.97e$-$02&2.77e$-$01&448 \\
374&249&\no&J172401+6543.6&\no&261.00535&65.72757&\no&\no&N&8.11e$-$01&1.00e+00&35 \\
375&4&12&J172401+6600.5&1&261.00660&66.00962&0.8918&\no&Q&7.93e$-$04&7.92e$-$01&1770 \\
376&\no&19&J172402+6538.3&91&261.00960&65.63860&\no&\no&N&7.73e$-$01&6.93e$-$01&281 \\
377&279&\no&J172403+6552.2&\no&261.01652&65.87056&\no&\no&N&9.88e$-$01&9.99e$-$01&42 \\
378&36&26&J172405+6550.5&8&261.02193&65.84259&\no&\no&N&6.57e$-$01&3.20e$-$01&336 \\
379&205&43&J172407+6543.9&14&261.03328&65.73184&\no&\no&G&9.50e$-$01&7.96e$-$01&135 \\
380&156&\no&J172408+6546.2&\no&261.03516&65.77165&\no&\no&N&8.91e$-$01&8.18e$-$01&60 \\
381&\no&158&J172408+6535.9&\no&261.03634&65.59940&\no&\no&N&9.77e$-$01&8.98e$-$01&37 \\
382&\no&225&J172408+6549.5&\no&261.03685&65.82599&\no&\no&G&7.92e$-$01&9.64e$-$01&50 \\
383&\no&152&J172409+6549.6&80&261.03899&65.82798&\no&\no&N&4.24e$-$01&7.66e$-$01&120 \\
384&\no&147&J172409+6552.1&\no&261.04011&65.86980&\no&\no&N&7.32e$-$01&9.76e$-$01&38 \\
385&86&\no&J172410+6549.5&\no&261.04296&65.82557&\no&\no&N&4.65e$-$01&9.42e$-$01&118 \\
386&57&71&J172410+6602.4&\no&261.04555&66.04058&\no&\no&N&4.84e$-$01&2.95e$-$01&240 \\
387&222&\no&J172411+6556.4&\no&261.04695&65.94050&\no&\no&N&1.00e+00&8.92e$-$01&49 \\
388&277&\no&J172411+6602.0&\no&261.04807&66.03468&\no&\no&N&7.28e$-$01&4.65e$-$01&46 \\
389&\no&163&J172411+6540.1&\no&261.04974&65.66834&\no&\no&N&8.21e$-$01&7.41e$-$01&107 \\
390&245&\no&J172412+6549.4&\no&261.05313&65.82489&\no&\no&N&9.83e$-$01&1.00e+00&38 \\
391&\no&100&J172412+6543.4&\no&261.05336&65.72360&\no&\no&N&9.95e$-$01&9.61e$-$01&38 \\
392&92&276&J172413+6555.4&\no&261.05641&65.92455&\no&\no&N&3.54e$-$01&8.67e$-$01&266 \\
393&\no&146&J172414+6547.1&\no&261.05941&65.78544&\no&0.29&N&9.43e$-$01&9.89e$-$01&42 \\
394&\no&160&J172414+6559.8&\no&261.06098&65.99768&\no&\no&N&9.86e$-$01&2.06e$-$01&63 \\
395&208&\no&J172415+6543.9&\no&261.06267&65.73203&\no&\no&N&9.72e$-$01&9.99e$-$01&53 \\
396&227&\no&J172415+6546.8&\no&261.06399&65.78113&\no&\no&N&7.40e$-$01&8.73e$-$01&38 \\
397&51&59&J172416+6548.8&11&261.06943&65.81464&0.3759&\no&G&5.56e$-$01&5.36e$-$01&198 \\
398&164&\no&J172416+6556.4&\no&261.06948&65.94002&\no&\no&N&6.55e$-$01&7.97e$-$01&54 \\
399&\no&123&J172417+6556.3&\no&261.07163&65.93840&\no&\no&N&7.83e$-$01&8.12e$-$01&114 \\
400&252&\no&J172417+6552.9&\no&261.07478&65.88187&\no&\no&N&9.94e$-$01&9.33e$-$01&50 \\
401&204&\no&J172418+6556.0&\no&261.07791&65.93490&\no&\no&N&9.78e$-$01&9.85e$-$01&59 \\
402&255&\no&J172419+6547.4&\no&261.08093&65.79100&\no&\no&N&1.00e+00&9.25e$-$01&58 \\
403&\no&150&J172419+6547.1&\no&261.08106&65.78509&\no&0.41&N&8.96e$-$01&9.62e$-$01&37 \\
404&187&\no&J172421+6605.5&\no&261.08941&66.09188&\no&\no&N&\no&\no&50 \\
405&95&62&J172421+6546.8&\no&261.08952&65.78118&\no&\no&N&8.78e$-$01&8.72e$-$01&153 \\
406&64&\no&J172421+6548.7&11&261.09036&65.81277&0.8371&\no&Q&4.96e$-$01&4.70e$-$01&116 \\
407&\no&167&J172421+6549.0&\no&261.09043&65.81818&\no&\no&N&8.06e$-$01&9.74e$-$01&51 \\
408&189&\no&J172426+6555.7&\no&261.11122&65.92893&\no&\no&N&8.79e$-$01&8.72e$-$01&46 \\
409&285&\no&J172426+6542.6&\no&261.11150&65.71038&\no&\no&N&9.83e$-$01&9.29e$-$01&42 \\
410&\no&159&J172429+6541.1&\no&261.12239&65.68626&\no&\no&N&3.38e$-$01&8.40e$-$02&77 \\
411&\no&112&J172429+6555.6&\no&261.12433&65.92810&\no&\no&N&9.62e$-$01&8.46e$-$01&59 \\
412&61&127&J172431+6546.7&84&261.12926&65.77892&\no&\no&N&3.94e$-$01&9.98e$-$01&211 \\
413&\no&56&J172431+6539.9&108&261.12964&65.66646&\no&\no&N&6.27e$-$01&5.75e$-$01&258 \\
414&266&\no&J172432+6545.6&\no&261.13741&65.76123&\no&\no&N&9.59e$-$01&9.97e$-$01&49 \\
415&172&\no&J172434+6559.9&\no&261.14466&65.99884&\no&\no&N&5.99e$-$01&9.67e$-$01&43 \\
416&154&186&J172435+6549.6&\no&261.14819&65.82814&0.0064&\no&G&3.57e$-$01&9.01e$-$01&147 \\
417&\no&201&J172436+6548.5&\no&261.15080&65.80866&\no&\no&N&8.67e$-$01&9.69e$-$01&37 \\
418&199&\no&J172436+6548.4&\no&261.15275&65.80726&\no&\no&N&3.67e$-$01&1.00e+00&31 \\
419&271&\no&J172437+6547.7&\no&261.15432&65.79639&\no&\no&N&1.00e+00&8.55e$-$01&39 \\
420&180&\no&J172439+6603.3&\no&261.16288&66.05642&\no&\no&N&\no&\no&41 \\
421&\no&195&J172440+6538.8&\no&261.16801&65.64701&\no&\no&N&2.60e$-$02&1.00e+00&107 \\
422&20&\no&J172441+6556.7&\no&261.17156&65.94645&\no&\no&N&3.20e$-$06&9.54e$-$01&196 \\
423&\no&136&J172441+6542.9&\no&261.17203&65.71562&\no&0.84&N&8.64e$-$01&4.72e$-$01&36 \\
424&\no&148&J172445+6541.0&\no&261.19028&65.68340&\no&\no&N&4.73e$-$01&2.48e$-$01&27 \\
425&\no&268&J172446+6541.9&104&261.19330&65.69865&\no&\no&N&6.16e$-$01&\no&58 \\
426&\no&154&J172446+6543.5&\no&261.19431&65.72639&\no&\no&N&8.35e$-$01&8.18e$-$01&33 \\
427&\no&196&J172449+6542.7&\no&261.20464&65.71298&\no&\no&N&9.04e$-$01&3.90e$-$01&25 \\
428&\no&219&J172450+6543.9&\no&261.20883&65.73298&\no&\no&N&4.57e$-$01&8.88e$-$01&65 \\
429&224&\no&J172450+6554.8&\no&261.20948&65.91401&0.8256&\no&G&3.21e$-$01&9.66e$-$01&35 \\
430&192&\no&J172452+6551.0&\no&261.21803&65.85159&\no&\no&N&1.00e+00&8.77e$-$01&50 \\
431&\no&264&J172453+6547.5&\no&261.22486&65.79229&\no&\no&N&9.52e$-$01&9.88e$-$01&36 \\
432&\no&92&J172454+6555.8&\no&261.22880&65.93009&\no&\no&N&1.00e+00&7.67e$-$01&51 \\
433&\no&18&J172455+6543.2&106&261.22926&65.72101&\no&0.39&N&8.79e$-$01&4.43e$-$01&240 \\
434&\no&232&J172455+6545.3&\no&261.23040&65.75640&\no&\no&N&9.03e$-$01&6.32e$-$01&36 \\
435&\no&274&J172456+6557.1&\no&261.23526&65.95220&\no&0.51&N&8.63e$-$01&8.19e$-$01&48 \\
436&\no&241&J172457+6556.3&\no&261.24039&65.93891&\no&\no&N&9.13e$-$01&4.80e$-$01&41 \\
437&210&\no&J172458+6558.6&\no&261.24186&65.97797&\no&\no&N&1.25e$-$01&9.56e$-$01&46 \\
438&\no&99&J172458+6552.9&\no&261.24465&65.88208&\no&\no&N&9.99e$-$01&6.04e$-$01&65 \\
439&\no&214&J172459+6547.7&\no&261.24905&65.79610&\no&\no&N&7.81e$-$01&7.75e$-$01&35 \\
440&\no&189&J172500+6549.9&\no&261.25052&65.83196&\no&\no&N&9.73e$-$01&9.63e$-$01&48 \\
441&\no&236&J172502+6557.6&\no&261.25910&65.96095&\no&\no&N&\no&4.73e$-$01&34 \\
442&174&\no&J172504+6551.8&\no&261.26847&65.86460&\no&\no&N&4.46e$-$01&6.06e$-$01&43 \\
443&265&\no&J172509+6547.0&\no&261.28785&65.78336&\no&\no&N&\no&3.40e$-$01&27 \\
444&\no&137&J172514+6554.9&\no&261.30994&65.91614&\no&\no&N&\no&6.34e$-$01&35 \\
445&\no&173&J172514+6551.8&\no&261.31192&65.86386&\no&\no&N&8.54e$-$01&8.91e$-$01&47 \\
446&\no&199&J172515+6550.9&\no&261.31269&65.84847&\no&\no&N&3.88e$-$01&7.93e$-$01&56 \\
447&\no&119&J172516+6553.4&\no&261.31914&65.89109&\no&\no&N&8.28e$-$01&6.34e$-$01&76 \\
448&\no&176&J172516+6549.5&\no&261.32053&65.82614&\no&\no&N&\no&7.27e$-$01&102 \\
449&\no&171&J172517+6547.7&\no&261.32149&65.79612&\no&\no&N&\no&\no&45 \\
450&\no&260&J172519+6548.0&\no&261.33156&65.80058&\no&\no&N&\no&\no&34 \\
451&\no&267&J172519+6549.2&\no&261.33317&65.82112&\no&\no&N&\no&\no&72 \\
452&\no&209&J172520+6552.0&\no&261.33339&65.86806&\no&\no&N&5.39e$-$01&\no&52 \\
453&\no&188&J172523+6552.4&\no&261.34905&65.87416&\no&\no&N&\no&\no&102 \\

